AutoDAN-Turbo: A Lifelong Agent for Strategy Self-Exploration to Jailbreak LLMs

In this paper, we propose AutoDAN-Turbo, a black-box jailbreak method that can automatically discover as many jailbreak strategies as possible from scratch, without any human intervention or predefined scopes (e.g., specified candidate strategies), and use them for red-teaming. As a result, AutoDAN-Turbo can significantly outperform baseline methods, achieving a 74.3% higher average attack success rate on public benchmarks. Notably, AutoDAN-Turbo achieves an 88.5 attack success rate on GPT-4-1106-turbo. In addition, AutoDAN-Turbo is a unified framework that can incorporate existing human-designed jailbreak strategies in a plug-and-play manner. By integrating human-designed strategies, AutoDAN-Turbo can even achieve a higher attack success rate of 93.4 on GPT-4-1106-turbo.

==> sections/saved-tables.tex <==
\begin{table}
  \caption{Self-jailbreaking}
  \label{self_jailbreak_results}
  \centering
  \small
\begin{tabular}{ccccc}
\toprule
Model              & Attack Success Rate ($ASR$) & \multicolumn{3}{c}{Total Strategies Found   ($TSF$)} \\ \cmidrule{3-5}
                   &                             & Singular   Strategies   & Mixed Strategies  & Total  \\ 

\midrule
Llama-2-7B-chat    & 27.49\%                     & 16                      & 5                 & 21     \\
Llama-2-13B-chat   & 30.66\%                     & 24                      & 18                & 42     \\
Llama-2-70B-chat   & 33.67\%                     & 32                      & 20                & 52     \\
Llama-3-8B         & 36.18\%                     & 26                      & 23                & 49     \\
Llama-3-70B        & 53.90\%                     & 37                      & 19                & 56     \\
Gemma-7b-it        & 42.91\%                     & 41                      & 33                & 74     \\
MixT5              & 31.46\%                     & 40                      & 7                 & 47     \\
gpt-4-0125-preview & 23.14\%                     & 35                      & 16                & 51     \\
gpt-4-1106-turbo   & 37.76\%                     & 30                      & 20                & 50     \\
Claude 2.0         & 1.44\%                      & 3                       & 1                 & 4      \\
Claude 2.1         & 1.01\%                      & 3                       & 0                 & 3      \\
Claude 3 Haiku     & 0.31\%                      & 2                       & 0                 & 2      \\
Claude 3 Sonnet    & 0.24\%                      & 2                       & 0                 & 2      \\
Claude 3 Opus      & 0.24\%                      & 2                       & 0                 & 2      \\
Gemini Pro         & 54.41\%                     & 39                      & 36                & 75 \\
\bottomrule
\end{tabular}
\end{table}		


\begin{table}
  \caption{Cross jailbreak}
  \label{sample-table}
  \centering
  \small
\begin{tabular}{cccccc}
\toprule
Attacker   ($A$) & Target ($T$) & Attack Success Rate ($ASR$) & \multicolumn{3}{c}{Total Strategies Found   ($TSF$)} \\ \cmidrule{4-6}
                 &                  &         & Singular Strategies & Mixed Strategies & Total \\
\midrule
Llama-2-7B-chat  & Llama-3-8B       & 51.40\% & 14                  & 6                & 20    \\
Llama-2-7B-chat  & Gemma-7b-it      & 31.38\% & 15                  & 6                & 21    \\
Llama-2-13B-chat & MixT5            & 31.10\% & 26                  & 5                & 31    \\
Llama-2-13B-chat & Gemma-7b-it      & 36.98\% & 34                  & 14               & 48    \\
Llama-2-70B-chat & Gemma-7b-it      & 36.24\% & 35                  & 18               & 53    \\
Llama-2-70B-chat & Llama-3-70B      & 66.63\% & 30                  & 21               & 51    \\
MixT5            & Gemma-7b-it      & 38.21\% & 41                  & 18               & 59    \\
MixT5            & Llama-2-13B-chat & 30.43\% & 34                  & 5                & 39    \\
Gemma-7b-it      & Llama-2-7B-chat  & 29.45\% & 41                  & 30               & 71    \\
Gemma-7b-it      & Llama-2-13B-chat & 33.67\% & 40                  & 28               & 68    \\
Gemma-7b-it      & Llama-2-70B-chat & 34.45\% & 42                  & 28               & 70    \\
Gemma-7b-it      & MixT5            & 34.61\% & 43                  & 23               & 66    \\
Gemma-7b-it      & Llama-3-8B       & 53.11\% & 36                  & 32               & 68    \\
Gemma-7b-it      & Llama-3-70B      & 54.48\% & 40                  & 31               & 71    \\
Llama-3-8B       & Gemma-7b-it      & 56.47\% & 38                  & 34               & 72    \\
Llama-3-8B       & Gemini Pro       & 61.17\% & 29                  & 31               & 60    \\
Llama-3-8B       & Llama-2-7B-chat  & 33.11\% & 40                  & 27               & 67    \\
Llama-3-70B      & Gemma-7b-it      & 65.16\% & 43                  & 33               & 76    \\
Llama-3-70B      & Llama-2-70B-chat & 34.10\% & 44                  & 31               & 75    \\
Llama-3-70B      & Gemini Pro       & 66.10\% & 34                  & 32               & 66    \\
Gemini Pro       & Llama-3-8B       & 62.48\% & 34                  & 30               & 64    \\
Gemini Pro       & Llama-3-70B      & 68.42\% & 37                  & 32               & 69    \\
Gemini Pro       & Claude 2.0       & 2.10\%  & 38                  & 33               & 71    \\
Claude 2.0       & Gemini Pro       & 8.81\%  & 3                   & 0                & 3     \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{Transfer Jailbreaking with Various Strategy Libraries ($SL$)}
  \label{sample-table}
  \centering
  \small
\begin{tabular}{c|ccccccccccc}
\toprule
\
 &
  gpt-4-1106-turbo &
  Llama-2-7B-chat &
  Llama-2-13B-chat &
  Llama-2-70B-chat &
  Llama-3-8B &
  Llama-3-70B &
  Gemma-7b-it &
  Gemini Pro &
  Claude 2.0 &
  Claude 2.1 &
  Claude 3 Opus \\ 
  \midrule
Llama-2-7B-chat &
  76.4/9.8/2.0 &
  27.5/10.4/4.1 &
  31.8/7.7/3.8 &
  33.4/9.4/4.6 &
  39.2/11.6/4.1 &
  41.3/11.6/5.2 &
  41.4/13.4/4.4 &
  48.0/13.7/4.2 &
  1.6/1.6/1.6 &
  0.8/0.8/0.8 &
  0.6/0.6/0.6 \\
Llama-2-13B-chat &
  74.1/9.7/2.6 &
  33.0/9.8/2.5 &
  31.2/8.9/4.1 &
  34.4/8.8/5.2 &
  40.0/12.6/5.9 &
  43.9/10.6/4.6 &
  46.4/12.5/4.0 &
  56.3/12.5/4.1 &
  2.0/2.0/2.0 &
  1.1/1.1/1.1 &
  0.6/0.6/0.6 \\
Llama-2-70B-chat &
  74.8/10.4/2.0 &
  32.2/12.5/3.2 &
  30.6/9.8/4.6 &
  33.8/9.9/4.2 &
  44.7/11.1/3.8 &
  47.5/9.3/4.0 &
  43.2/11.6/5.0 &
  58.8/11.5/5.3 &
  2.3/2.3/2.3 &
  1.1/1.1/1.1 &
  0.8/0.8/0.8 \\
Llama-3-8B &
  80.6/10.9/2.9 &
  32.7/11.9/4.1 &
  32.4/8.8/5.2 &
  44.7/10.9/4.1 &
  52.8/12.8/4.2 &
  54.7/9.8/3.8 &
  60.4/9.8/4.6 &
  60.4/11.3/4.3 &
  2.3/2.3/2.31 &
  1.1/1.1/1.1 &
  1.0/1.0/1.0 \\
Llama-3-70B &
  82.6/10.4/2.0 &
  33.4/10.5/4.1 &
  31.9/9.4/4.1 &
  41.2/11.1/5.0 &
  57.0/11.3/4.2 &
  58.8/11.2/4.1 &
  61.3/10.6/3.8 &
  64.4/12.3/5.2 &
  2.6/2.6/2.6 &
  1.8/1.8/1.8 &
  0.8/0.8/0.8 \\
Gemma-7b-it &
  79.4/11.2/2.9 &
  33.0/11.3/3.1 &
  34.4/10.0/4.6 &
  42.6/9.4/5.2 &
  50.6/10.9/3.0 &
  56.8/12.0/5.3 &
  62.8/8.8/4.2 &
  62.2/12.7/4.1 &
  2.5/2.5/2.5 &
  1.5/1.5/1.5 &
  1.5/1.5/1.5 \\
Gemini Pro &
  81.9/12.5/4.9 &
  33.8/11.6/5.0 &
  34.6/13.1/5.2 &
  43.2/13.3/4.2 &
  53.0/11.6/4.0 &
  57.3/13.6/5.3 &
  58.8/13.1/4.2 &
  63.2/10.8/4.0 &
  1.9/1.9/1.9 &
  1.3/1.3/1.3 &
  1.1/1.1/1.1
\end{tabular}

\end{table}

\begin{table}
  \caption{Llama-Guard Built-in Jailbreaking Methods (black-box) Comparison}
  \label{sample-table}
  \centering
  \small
  \begin{tabular}{ccccc}
  \toprule
Method & Attacker ($A$) & Target ($T$) & Attack Success Rate Under   Llama-Guard-7B ($Guard-7B-ASR$) & Attack Success Rate Under   Llama-Guard-2-8B ($Guard-2-8B-ASR$) \\
\midrule
GCG-T      & Llama-2-7B-chat  & Llama-2-7B-chat  & 5.61\%  & 3.44\% \\
PAIR       & Llama-2-7B-chat  & Llama-2-7B-chat  & 2.46\%  & 0.22\% \\
TAP        & Llama-2-7B-chat  & Llama-2-7B-chat  & 3.08\%  & 0.28\% \\
PAP-top5   & Llama-2-7B-chat  & Llama-2-7B-chat  & 4.11\%  & 1.12\% \\
Our Method & Llama-2-7B-chat  & Llama-2-7B-chat  & 14.48\% & 8.86\% \\
GCG-T      & Llama-2-13B-chat & Llama-2-13B-chat & 4.11\%  & 2.24\% \\
PAIR       & Llama-2-13B-chat & Llama-2-13B-chat & 2.52\%  & 0.33\% \\
TAP        & Llama-2-13B-chat & Llama-2-13B-chat & 2.20\%  & 0.28\% \\
PAP-top5   & Llama-2-13B-chat & Llama-2-13B-chat & 2.26\%  & 0.33\% \\
Our Method & Llama-2-13B-chat & Llama-2-13B-chat & 12.53\% & 5.92\% \\
GCG-T      & Llama-2-70B-chat & Llama-2-70B-chat & 6.68\%  & 3.54\% \\
PAIR       & Llama-2-70B-chat & Llama-2-70B-chat & 2.20\%  & 0.22\% \\
TAP        & Llama-2-70B-chat & Llama-2-70B-chat & 2.20\%  & 1.12\% \\
PAP-top5   & Llama-2-70B-chat & Llama-2-70B-chat & 2.26\%  & 0.33\% \\
Our Method & Llama-2-70B-chat & Llama-2-70B-chat & 13.61\% & 5.42\% \\
GCG-T      & Llama-3-8B       & Llama-3-8B       & 6.68\%  & 2.52\% \\
PAIR       & Llama-3-8B       & Llama-3-8B       & 3.23\%  & 1.12\% \\
TAP        & Llama-3-8B       & Llama-3-8B       & 3.08\%  & 1.43\% \\
PAP-top5   & Llama-3-8B       & Llama-3-8B       & 2.92\%  & 1.92\% \\
Our Method & Llama-3-8B       & Llama-3-8B       & 14.11\% & 5.61\% \\
GCG-T      & Llama-3-70B      & Llama-3-70B      & 8.42\%  & 3.23\% \\
PAIR       & Llama-3-70B      & Llama-3-70B      & 4.11\%  & 1.92\% \\
TAP        & Llama-3-70B      & Llama-3-70B      & 4.86\%  & 1.12\% \\
PAP-top5   & Llama-3-70B      & Llama-3-70B      & 3.08\%  & 1.92\% \\
Our Method & Llama-3-70B      & Llama-3-70B      & 14.73\% & 9.71\% \\
GCG-T      & MixT5            & MixT5            & 7.83\%  & 3.54\% \\
PAIR       & MixT5            & MixT5            & 5.92\%  & 1.43\% \\
TAP        & MixT5            & MixT5            & 5.58\%  & 1.43\% \\
PAP-top5   & MixT5            & MixT5            & 4.42\%  & 1.12\% \\
Our Method & MixT5            & MixT5            & 13.64\% & 5.92\% \\
GCG-T      & Gemma-7b-it      & Gemma-7b-it      & 5.61\%  & 2.92\% \\
PAIR       & Gemma-7b-it      & Gemma-7b-it      & 3.08\%  & 1.43\% \\
TAP        & Gemma-7b-it      & Gemma-7b-it      & 4.41\%  & 1.12\% \\
PAP-top5   & Gemma-7b-it      & Gemma-7b-it      & 3.23\%  & 1.41\% \\
Our Method & Gemma-7b-it      & Gemma-7b-it      & 12.53\% & 5.58\% \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[]
  \caption{Transfer Jailbreak Strategy Learning with A Same Target ($T$)}
  \label{sample-table}
  \centering
  \small
\begin{tabular}{ccccccc}
\toprule
Attacker   ($A$) &
  Strategy Library ($SL$) &
  Target ($T$) &
  Previous Attack Success Rate   ($Pre-ASR$) &
  Previous Total Strategies Found   ($Prev-TSF$) &
  Post Attack Success Rate   ($Post-ASR$) &
  Post Total Strategies Found   ($Post-TSF$) \\
  \midrule
Gemma-7b-it      & Llama-2-7B-chat  & Llama-3-8B & 44.50\% & 21 & 54.46\% & 32 \\
Llama-2-7B-chat  & Gemma-7b-it      & Llama-3-8B & 46.62\% & 74 & 47.25\% & 74 \\
Gemma-7b-it      & Llama-2-13B-chat & Llama-3-8B & 57.30\% & 42 & 61.17\% & 49 \\
Llama-2-13B-chat & Gemma-7b-it      & Llama-3-8B & 51.40\% & 74 & 53.49\% & 74 \\
Gemma-7b-it      & Llama-2-70B-chat & Llama-3-8B & 56.70\% & 52 & 62.48\% & 58 \\
Llama-2-70B-chat & Gemma-7b-it      & Llama-3-8B & 54.46\% & 74 & 55.80\% & 74 \\
Gemma-7b-it      & Llama-3-8B       & Llama-3-8B & 57.30\% & 49 & 62.48\% & 57 \\
Llama-3-8B       & Gemma-7b-it      & Llama-3-8B & 60.48\% & 74 & 61.60\% & 74 \\
Gemma-7b-it      & Llama-3-70B      & Llama-3-8B & 58.10\% & 56 & 61.18\% & 59 \\
Llama-3-70B      & Gemma-7b-it      & Llama-3-8B & 61.46\% & 74 & 62.48\% & 74 \\
Llama-3-70B      & Llama-3-8B       & Llama-3-8B & 58.10\% & 49 & 62.32\% & 50 \\
Llama-3-8B       & Llama-3-70B      & Llama-3-8B & 58.48\% & 56 & 61.60\% & 56 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\caption{Transfer Jailbreak Strategy Learning with Different Target ($T$) (Control Group) }
  \label{sample-table}
  \centering
  \small
\begin{tabular}{ccccccc}
\toprule
Attacker   ($A$) &
  Strategy Library ($SL$) &
  Target ($T$) &
  Previous Attack Success Rate   ($Pre-ASR$) &
  Previous Total Strategies Found   ($Prev-TSF$) &
  Post Attack Success Rate   ($Post-ASR$) &
  Post Total Strategies Found   ($Post-TSF$) \\
\midrule
Gemma-7b-it     & Llama-2-7B-chat & Llama-3-8B       & 44.50\% & 21 & 54.46\% & 32 \\
Gemma-7b-it     & Llama-2-7B-chat & Llama-3-70B      & 54.48\% & 21 & 56.70\% & 33 \\
Gemma-7b-it     & Llama-2-7B-chat & Llama-2-7B-chat  & 31.10\% & 21 & 33.11\% & 25 \\
Gemma-7b-it     & Llama-2-7B-chat & Llama-2-13B-chat & 33.11\% & 21 & 33.91\% & 28 \\
Llama-2-7B-chat & Gemma-7b-it     & Llama-3-8B       & 46.62\% & 74 & 47.25\% & 74 \\
Llama-2-7B-chat & Gemma-7b-it     & Llama-3-70B      & 53.68\% & 74 & 54.63\% & 74 \\
Llama-2-7B-chat & Gemma-7b-it     & Llama-2-7B-chat  & 28.43\% & 74 & 28.91\% & 74 \\
Llama-2-7B-chat & Gemma-7b-it     & Llama-2-13B-chat & 32.71\% & 74 & 33.41\% & 74 \\
\bottomrule
\end{tabular}
\end{table}


